Concepts Rookie Book

This book begins with the basic accelerator knowledge required to understand the latter chapters. This is followed by topics from Fermilab accelerator specifics to general accelerator physics concepts. These chapters are accompanied by descriptions of the instrumentation and utilities required to operate a high-energy physics laboratory. Last, we discuss the role of operators in safety at the lab.

==> definitions.tex <==
%%                              %%
%%     Keyterm Definitions      %%
%%                              %%

\newglossaryentry{acceleration}
{
  name=acceleration,
  description={is the act of increasing the kinetic energy of a particle beam}
}
\newglossaryentry{bucket}
{
	name=bucket,
	description={is the set of particle energies and phases that can be captured and accelerated by the RF. This is equivalent to an area in longitudinal phase space}
}
\newglossaryentry{beam}
{
  name=beam,
  description={is a focused group of particles all traveling in the same overall direction}
}
\newglossaryentry{bunch}
{
  name=bunch,
  description={is the beam within a bucket; think of it as a cloud of particles},
  plural={bunches}
}
\newglossaryentry{harmonicnumber}
{
  name=harmonic number,
  description={is the number of times the RF field oscillates in one beam orbit of a circular machine. This is equivalent to the number of RF buckets in a machine, and thus the maximum number of bunches an accelerator. It can be calculated by multiplying the beam revolution period by the RF frequency}
}
\newglossaryentry{batch}
{
  name=batch,
  description={is the full output of one Booster cycle, which is equivalent to 84 bunches},
  plural=batches
}
\newglossaryentry{multibatch}
{
  name=multi-batch,
  description={is the process of sending two or more consecutive batches to the Recycler/Main Injector},
  plural=multi-batching
}
\newglossaryentry{partialbatch}
{
  name=partial-batch,
  description={is the process of sending a portion of a full batch to Recycler/Main Injector/BNB},
  plural=partial-batching
}
\newglossaryentry{injection}
{
  name=injection,
  description={is the process of placing beam into an accelerator},
  plural=injections
}
\newglossaryentry{extraction}
{
  name=extraction,
  description={is the process of removing beam from an accelerator},
  plural=extractions
}
\newglossaryentry{btobtransfer}
{
  name=bucket-to-bucket transfer,
  description={is the process of placing injected beam into RF buckets},
  plural=bucket-to-bucket transfers
}
\newglossaryentry{transfercogging}
{
  name=transfer cogging,
  description={is when a downstream machine matches its RF phase to an upstream machine during bucket-to-bucket transfers},
}
\newglossaryentry{turn}
{
  name=turn,
  description={A turn is one circumference of Booster beam. Multiple turns means that injected beam is combined with already-circulating beam; the more turns, the higher the beam intensity. We control the number of turns by changing the pulse length of the beam injected into Booster}
}
\newglossaryentry{transverse}
{
  name=transverse,
  description={refers to the horizontal or vertical plane, perpendicular to the direction of beam travel}
}
\newglossaryentry{longitudinal}
{
  name=longitudinal,
  description={is parallel to the direction that beam travels}
}
\newglossaryentry{emittance}
{
  name=emittance,
  description={is a beam parameter related to the size of particle betatron or synchrotron oscillations. This involves the oscillation amplitude (transverse displacement or longitudinal phase) and the derivative thereof}
}
\newglossaryentry{synchrotron}
{
  name=synchrotron,
  description={is a circular accelerator that guides beam on a closed obit to allow a small set of RF cavities to accelerate beam over many revolutions. The dipole magnetic field and RF frequency must be increase together for controlled acceleration}
}
\newglossaryentry{dipole}
{
  name=dipole,
  description={has two pole faces that create a magnetic field which bends beam horizontally or vertically}
}
\newglossaryentry{bump}
{
  name=bump,
  description={is 3 or more dipoles creating a beam position or angle change in a specific area without affecting the rest of the orbit}
}
\newglossaryentry{dispersion}
{
  name=dispersion,
  description={is the way in which beam momentum spread leads to a transverse deviation from the ideal orbit. This is due to the velocity-dependent nature of the magnetic field: low-momentum particles are bent more than high-momentum}
}
\newglossaryentry{quadrupole}
{
  name=quadrupole,
  description={has four pole faces that create a magnetic field which focuses the beam, like a lens, in one transverse plane but defocuses beam in the other. Quads are arranged in a repeating alternating pattern known as a lattice, and control the tune of an accelerator. Quadrupoles provide the restoring force that causes betatron oscillation}
}
\newglossaryentry{betatronoscillation}
{
  name=betatron oscillation,
  description={is the transverse oscillation around the ideal orbit, and is due to the restoring force provided by the quadrupole magnets}
}
\newglossaryentry{lattice}
{
  name=lattice,
  description={is the arrangement of an accelerators quadrupole magnets into a periodic pattern. In a synchrotron this involves the repetition of alternating focusing and defocusing quads}
}
\newglossaryentry{cell}
{
  name=cell,
  description={is the smallest repeating pattern in a lattice}
}
\newglossaryentry{tune}
{
  name=tune,
  description={is the number of betatron oscillations per beam revolution. The tune is controlled with the quadrupole magnet lattice}
}
\newglossaryentry{chromaticity}
{
  name=chromaticity,
  description={is the effect that beam momentum spread has on the tune spread. This is due to the velocity-dependent nature of the magnetic field: for a given quadrupole, low-momentum particles have a lower focal length than high-momentum particles. Chromaticity can be controlled with sextupole magnets},
  plural={chromaticities}
}
\newglossaryentry{sextupole}
{
  name=sextupole,
  description={have six pole faces. Sextupoles control the chromaticity by compensating for the momentum-dependence of quadrupole focusing}
}
\newglossaryentry{octupole}
{
  name=octupole,
  description={have eight pole faces. Octupoles can control the tune spreads dependence on particle betatron oscillation amplitude}
}
\newglossaryentry{chopper}
{
  name=chopper,
  description={is a device used to deflect a portion of a continuous stream of beam}
}
\newglossaryentry{kicker}
{
  name=kicker,
  description={is a pulsed magnet whose field can rise and fall very quickly. In conjunction with a Lambertson or septum magnet, kickers are used to either place beam onto a closed orbit (injection) or to take beam off a closed orbit (extraction)}
}
\newglossaryentry{Lambertson}
{
  name=Lambertson,
  description={a type of septum magnet, is a magnet with at least two separate apertures. One aperture, called the field-free region, does not deflect the beam.  The other aperture, called the field region, acts as a dipole.  This is commonly used during the injection or extraction process to bend beam towards or away from a circulating path, respectively}
}
\newglossaryentry{RFcavity}
{
  name=RF cavity,
  description={is a resonant structure that efficiently produces a standing electromagnetic wave.  The oscillating electric fields produced in these cavities capture or accelerate the beam},
  plural={RF cavities}
}
\newglossaryentry{phase}
{
  name=phase,
  description={is the difference between the timing of the RF cycle and a particle arrival time in the RF cavity. In other words, an incoming particle arrives at a certain point (phase) in the RF waveform due to the timing of when it arrives in the cavity}
}
\newglossaryentry{synchronousphase}
{
  name=synchronous phase,
  description={is the particle phase around which the accelerator is designed, and provides stable particle acceleration}
}
\newglossaryentry{phasefocusing}
{
  name=phase focusing,
  description={is the process that drives off-momentum or mistimed particles into stable longitudinal oscillations about the Synchronous Phase. Phase focusing provides the restoring force that causes synchrotron oscillations}
}
\newglossaryentry{synchrotronoscillation}
{
  name=synchrotron oscillation,
  description={is a longitudinal oscillation about the synchronous phase. This is due to the phase focusing process from the restoring force of the RF electric field}
}
\newglossaryentry{paraphasing}
{
  name=paraphasing,
  description={is the process where the Booster RF cavities, initially out of phase with one another, are slowly phased together after injection in order to capture 37.8-MHz bunches out of injected Linac beam}
}
\newglossaryentry{slipstacking}
{
  name=slip-stacking,
  description={is an RF beam manipulation performed to combine bunches to effectively double beam intensity}
}
\newglossaryentry{transition}
{
  name=transition,
  description={is a relativistic effect in synchrotrons where particle path length begins to have more of an effect on transit time than particle velocity. This occurs at the transition energy, and requires a synchronous phase flip to maintain RF phase focusing.}
}
\newglossaryentry{transitionenergy}
{
  name=transition energy,
  description={},
  plural={transition energies}
}
\newglossaryentry{separatrix}
{
  name=separatrix,
  description={is the boundary of the bucket area in phase space. Particles outside the separatrix undergo unstable motion and cannot be captured by the RF},
  plural={separatricies}
}
\newglossaryentry{magnet}
{
  name=magnet,
  description={}
}
\newglossaryentry{ramping}
{
  name=ramping,
  description={the magnets refers to increasing magnetic field to keep the bend radius of the beam path constant through acceleration}
}
\newglossaryentry{combinedfunctionmagnet}
{
  name=combined-function magnet,
  description={perform the roles of focusing and bending beam simultaneously}
}
\newglossaryentry{synchronousparticle}
{
  name=synchronous particle,
  description={arrives in the RF cavity at the synchronous phase, and is accelerated perfectly according to the accelerator design}
}
\newglossaryentry{ferritetuner}
{
  name=ferrite tuner,
  description={are small coaxial waveguides loaded with ferrite that change the resonant frequency of RF cavities in synchrotrons}
}
\newglossaryentry{failsafe}
{
  name=fail-safe,
  description={is a condition for a system in which if any of the parts are in an unknown state or fail the system is disabled in a safe manner}
}
\newglossaryentry{resonantextraction}
{
  name=resonant extraction,
  description={is a process that causes beam to fall out of the Main Injector in a slow controlled extraction, providing a long pulse of low-intensity beam for Switchyard.}
}
\newglossaryentry{electrostaticseptum}
{
  name=electrostatic septum,
  description={is a device that uses electric fields to split beam into multiple streams, either for sending beam to multiple beamlines in Switchyard, or to facilitate resonant extraction out of MI.}
}
\newglossaryentry{idealorbit}
{
  name=ideal orbit,
  description={is the path of the beam through the center of the magnets. In a synchrotron, the synchronous particle travels on the ideal orbit.}
}
\newglossaryentry{closedorbit}
{
  name=closed orbit,
  description={is the beam path that returns to the same point on every revolution around a circular machine. It is the beam trajectory which includes intentional bumps and corrections.}
}

%%                              %%
%%           Acronyms           %%
%%                              %%

\newacronym{bpm}{BPM}
{Beam Position Monitor}
\newacronym{bbm}{BBM}
{Beam Budget Monitor}
\newacronym{scl}{SCL}
{Side-Coupled Linac}
\newacronym{dtl}{DTL}
{Drift Tube Linac}
\newacronym{mta}{MTA}
{Muon Test Area}
\newacronym{rfq}{RFQ}
{Radio-frequency Quadrupole}
\newacronym{scr}{SCR}
{Silicon-Controlled Rectifier}
\newacronym{loto}{LOTO}
{Lockout/Tagout}
\newacronym{ess}{ESS}
{Electrical Safety System}
\newacronym{cdc}{CDC}
{Critical Device Controller}
\newacronym{tclk}{TCLK}
{Tevatron Clock}
\newacronym{ntf}{NTF}
{Neutron Therapy Facility}
\newacronym{bnb}{BNB}
{Booster Neutrino Beam}
\newacronym{lebt}{LEBT}
{Low Energy Beam Transport}
\newacronym{mebt}{MEBT}
{Medium Energy Beam Transport}
\newacronym{nova}{NO$\nu$A}
{NuMI Off-Axis $v_e$ Appearance}
\newacronym{minos}{MINOS}
{Main Injector Neutrino Oscillation Search}
\newacronym{minerva}{MINER$\nu$A}
{Main INjector ExpeRiment for $\nu$-A}
\newacronym{numi}{NuMI}
{Neutrinos at the Main Injector}
\newacronym{lrf}{LRF}
{LE Linac RF}
\newacronym{krf}{KRF}
{Klystron RF}
\newacronym{brf}{BRF}
{Booster RF}
\newacronym{rpos}{RPOS}
{Radial Position}
\newacronym{blm}{BLM}
{Beam Loss Monitor}
\newacronym{ipm}{IPM}
{Ion Profile Monitor}
\newacronym{odh}{ODH}
{Oxygen Deficiency Hazard}
\newacronym{dcct}{DCCT}
{DC Current Transformer}
\newacronym{mi}{MI}
{Main Injector}
\newacronym{mcr}{MCR}
{Main Control Room}
\newacronym{doe}{DOE}
{Department of Energy}
\newacronym{fnal}{FNAL}
{Fermi National Accelerator Laboratory}
\newacronym{nfpa}{NFPA 70E}
{National Fire Protection Association 70E}
\newacronym{esh}{ESH}
{Environmental, Safety, and Health Department}
\newacronym{rso}{RSO}
{Radiation Safety Officer}
\newacronym{cub}{CUB}
{Central Utility Building}
\newacronym{lcw}{LCW}
{Low Conductivity Water}
\newacronym{tsp}{TSP}
{Titanium Sublimation Pump}
\newacronym{rf}{RF}
{Radio Frequency}
\newacronym{dds}{DDS}
{Direct Digital Synthesizer}
\newacronym{ad}{AD}
{Accelerator Division}
\newacronym{llrf}{LLRF}
{Low-level RF}
\newacronym{hlrf}{HLRF}
{High-level RF}
\newacronym{pa}{PA}
{Power Amplifier}
